A Mixed Hierarchical Attention based Encoder-Decoder Approach for Standard Table Summarization

Structured data summarization involves generation of natural language summaries from structured input data. In this work, we consider summarizing structured data occurring in the form of tables as they are prevalent across a wide variety of domains. We formulate the standard table summarization problem, which deals with tables conforming to a single predefined schema. To this end, we propose a mixed hierarchical attention based encoder-decoder model which is able to leverage the structure in addition to the content of the tables. Our experiments on the publicly available WEATHERGOV dataset show around 18 BLEU (~ 30%) improvement over the current state-of-the-art.

==> model_old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% model details
\section{Tabular Data Summarization}
% In this section, we formulate the problem of \emph{standard table summarization} followed by description of the solution approaches in detail. 
A standard table consist of set of records (or rows) $ R = (r_{1}, r_{2},...r_{T})$ and each record $r$ has a fixed set of attributes (or columns) $ A^{r} = (a_{r1},a_{r2},...a_{rM})$. For the table shown in figure \ref{fig:standard_table}, there are 7 columns (apart from `TYPE') which correspond to different attributes. Also $U = (u_1, u_2,...u_T)$ represents the type of each record where $u_k$ is one-hot encoding for the record type for record $r_k$. Training data consists of instance pairs $(X_i, Y_i)$ for $i = 1,2,..n$, where $X_i=(R_i, U_i)$ represents the input table and $Y_i=(y_1,...,y_{T'})$ represents the corresponding natural language summary. In this paper, we propose an end-to-end model which takes in a table instance $X$ to produce the output summary $Y$. This can be derived by solving in ${Y}$ the following conditional probability objective:
\begin{align}
\label{eq0}
Y^*  &= \arg\max_{Y} \prod_{t=1}^{T'} p(y_t| y_1, ..., y_{t-1}, X)
\end{align}



% \subsection{Encoder-Decoder based Model}
% Decoder output $y_t$ and representation $h_t$ at time step $t$ can be described as,
% Encoder function can be expressed as,
% \begin{gather*}
% c = ENC(x_1,...,x_T)
% \end{gather*} 
% The decoder predicts sequence of output symbols $\textbf{y} = (y_1,...,y_{T'})$ using input vector $c$ and the 
% Decoder output $y_t$ and representation $h_t$ at time step $t$ can be described as,
% \begin{gather*}
%   y_t, h_t = DEC([y_{t-1}, c] , h_{t-1})
% \end{gather*}
%An RNN is a neural network which takes a sequence of input $\textbf{x} = (x_1,...,x_T)$ and produces a hidden representation $h_t$ at each time step $t$, where $h_t$ is the hidden state at time $t$ representing all previous inputs seen by the RNN. Given the current input symbol $x_t$ at time $t$ and previous hidden state $h_{t-1}$, hidden representation $h_t$ and output $y_t$ at time step $t$ can be calculated as follows,

%\begin{gather*}
%  h_t = f(W_{h} h_{t-1} + W_{x} x_{t}) \\
% y_t = o(W h_t)
%end{gather*}

%Here, the functions $f$ and $o$ denote some non-linear activations.
%Although RNNs can theoretically capture long term dependencies, they often suffer from exploding gradients and vanishing gradient problems. Gated recurrent unit (GRU) \cite{cho2014learning} is a variant which is easier to train and can capture long term dependencies by overcoming the above problems. GRU contains update and reset gates, which gives it flexibility to choose which information to keep and which one to skip. Given current input symbol $x_t$ and previous hidden state $h_{t-1}$, a GRU cell computes the new hidden state $h_t$ as defined below,
%\begin{gather*}
%z_t = \sigma(W_{z}x_t + V_z h_{t-1}) \\
%_t = \sigma(W_{r}x_t + V_r h_{t-1}) \\
%\tilde{h_t} = tanh(r_t \odot V h_{t-1} + W x_t)\\
%h_t = (1 - z_t) \odot \tilde{h_t} + z_t \odot h_{t-1} \\
%\end{gather*}

\begin{figure}[th] 
\centering
  \includegraphics[width=0.9\linewidth,keepaspectratio]{images/arch_half.png}
  \caption{Proposed Architecture}
  \label{fig:model_arch}
\end{figure}




\subsection{Mixed Hierarchical Attention Model (MHAM)}
Our model is based on the encode-attend-decode paradigm as defined in \cite{attn15}. It consists of an encoder RNN  which encodes a variable length input sequence $\textbf{x} = (x_1,...,x_T)$ into a representation sequence $\textbf{c}=(c_1,...,c_T)$. Another decoder RNN generates sequence of output symbols $\textbf{y} = (y_1,...,y_{T'})$, attending to different combinations of $c_i$ while generating different $y_t$.

As illustrated in figure \ref{fig:model_arch}, our encoder is not a single RNN. The encoder has a hierarchical structure to leverage the structural aspect of a \emph{standard table}: a table consists of a set of records (or rows) and each record consists of values corresponding to a fixed set of attributes. We call it a \emph{mixed hierarchical attention} based encoder, as it incorporates static attention and dynamic attention at two different levels of the encoder. At record level, the attention over record representations is \emph{dynamic} as it changes with each decoder time step.  Whereas at attribute level, since the schema is fixed, a record representation can be computed without the need of varying attention over attributes - thus \emph{static} attention. For example, with respect to \textsc{weathergov} dataset, a \emph{temperature} record will always be defined by the attributes like min, max and mean irrespective of the decoder time step. So, attention over attributes can be static. On the other hand, for while generating a word at decoder, there can be a preference of focussing on record type \emph{temperature} over some other type say, \emph{windSpeed}. Thus, dynamic attention over records.
	
% \paragraph*{Input Encodings:} If attribute types of the table are known as in the problem of fixed-schema, we can use specific encodings instead of simple one-hot vector representations. For example, we can use ordinal encodings for ordered attributes like time of day or direction and binary encodings for numbers depending on the range.
	
\paragraph*{Capturing attribute semantics:}
Typically the record type of a record provides substantial information about the values, specially in the context of how to talk about them. We use this motivation to specifically learn record type embeddings and use them to calculate attentions for a record. Given attributes $A^{r}$ for a record $r$, we embed each attribute:
%\begin{normalsize}
	\begin{align}
	\scriptstyle
	\bar{A_{j}^{r}} = W_jA_{j}^{r},\ \forall j \in [1,M]
	\end{align}
%	\end{normalsize}
	where $W_j$ is the embedding matrix for $j^{th}$ attribute. We embed record type vector through $W_0$ and project each attribute over corresponding record type as,
	\begin{align} \label{attr_projection}
	\bar{u_r} = W_0 \cdot u_r \\
	I^{r}_{j} = \bar{A_{j}^{r}} \bar{u_{r}}
	\end{align}
	
% \begin{figure*}[th] 
%   \includegraphics[width=\linewidth,keepaspectratio]{images/arch.png}
%   \caption{Proposed Architecture}
%   \label{fig:model_arch}
% \end{figure*}

\paragraph*{Static Attribute attention:}
	Not all attribute values contribute equally to the record. Hence, we introduce static attention weights for attributes of each record. We calculate attention probabilities $\alpha_{j}^{r}$ over attributes projected over corresponding record type vector (\ref{attr_projection}). The attention weights can then be used to calculate the record representation $B^r$ for record $r$. Specifically,
	
\begin{align}
	\alpha_{j}^{r} = softmax_j(I^r)\\
	B^r = \sum\limits_{j} \alpha_{j}^{r}  A_{j}^{r} 
\end{align}
	
	\paragraph*{Record Encoder:}
	%We use GRU \cite{gru} to encode attribute attended list of records,
	Our model uses a GRU based RNN encoder that takes as input a sequence of attribute attended records, represented as $B^{1:N} = (B^{1},B^{2},...,B^{N})$. It returns a sequence of hidden states $h_{1:N} = (h_{1},h_{2}...h_{N})$, where $h_{r}$ is the encoded summary for record $B^r$. 
	Given attribute attended list of records we get a record encoding using a GRU,
	\begin{align}
	{h_r} = GRU(B^r) \\
	c_r = \left[h_r;B^r\right]
	\end{align}
	We obtain the final record encoding $c_r$ by concatenating the GRU hidden stated with the embedded record encodings.
	\paragraph*{Static Record attention:} 
	In a table, a subset of records can always be more salient irrespective of the presence of other record types. This is captured by learning a static set of weights over all the records. These weights regulate the dynamic attention weights computed during decoding at each time step. Specifically,
	\begin{align*}
	g_r = \sigma(q^Ttanh(Pc_r))
	\end{align*}
	where, $g_r$ is the static record attention weight for $r^{th}$ record and $q$ and $P$ are weights to be learnt. We do not have any constraints on static attention vector. The idea behind not having any constraints or regularization is that it enables the model to be free not to have static record attention at all. This is helpful in cases where a rare combination of records appear in the input or a large number of records have interesting information to be summarized.
	\paragraph*{Dynamic Record attention for Decoder:}
	Our decoder is a GRU based decoder with dynamic attention mechanism, as the attention weights change for every decoder time step. At each time step $t$ of decoding, attention weights are calculated over the sequence of input records, based on which an output summary word at that time step is predicted. This attention mechanism is similar to \cite{weather16} with modifications to modulate attention weights at each time step using static record attentions. We calculate the attention weights as follows: 

	\begin{gather*}
	\beta^r_t = v^{T} tanh(W_{s}s_{t-1} + W_c c_{r}) \\
	w^r_{t} = softmax_r(\beta_t)\\
	%w^r_{t} = exp(\beta^r_{t})/\sum\limits_{j}exp(\beta^r_{t})\\
	\gamma^r_{t} = \frac{g_rw^r_{t}}{\sum\limits_{r}g_rw^r_{t}}\\
	\end{gather*}	
	Here, $\gamma^r_{t}$ is the final attention weight of record $r$ at time step $t$. We use the soft attention over input encoder sequences $c_r$ to calculate the weighted average, which is passed to the GRU. GRU outputs are used to calculate output probabilities by using a softmax as below,
	
	\begin{gather*}
	z_t = \sum\limits_{r}\gamma^r_{t}c_r\\
	s_t = GRU(z_t, s_{t-1})\\
	l_t = W_{1}s_{t} + W_{2}z_{t} + b_l\\
	p_t = softmax(l_t)
	\end{gather*}
	$p_t$ contains the probabilities at time step $t$ for each word in the vocabulary, based on which the output word $o_t$ is produced. 
	
Due to the static attention at attribute level, the time complexity of a single pass $O(TM + TT')$, where $T$ is the number of records, $M$ is the number of attributes and $T'$ is the number of decoder steps. In case of dynamic attention at both levels (as in \newcite{bowen16}), the time complexity is much higher $O(TMT')$. Thus, \emph{mixed hierarchical attention} model is faster than fully dynamic hierarchical attention. In addition to our proposed MHAM, for better understanding of the contribution of hierarchical attention, we propose a simpler architecture which is non-hierarchical (henceforth, NHM) as it will have attention only at record level.
	
%	\includegraphics[width=\textwidth,keepaspectratio]{images/arch.png}

%\subsection{Non-hierarchical model}
%We now describe the non-hierarchical model and the differences with the model proposed in \cite{weather16}. Our non-hierarchical model also had significant differences which gave a huge boost in performance in the first place. We concatenated the learned embedded vectors of with the encoder hidden representation instead of raw one-hot vector. We do not preform any regularization during training on GRU cells or on learned decoder attentions. Moreover, we dropped the constraints on global attention vector. Idea behind dropping these constraints is that in this case model is free not to have global attention at all. This will be helpful in cases where large number of records have interesting information to be summarized and can generalize to pick records which occurs rarely. In this model we used the ordinal encodings for attributes as described in section \ref{data-preprocess}. We used uni-directional GRU cells instead of bidirectional LSTM cells, which is a simpler to compute \cite{cho2014learning}.
	



==> problem.tex <==
	\section{Tabular Data Summarization} \label{Tabular Data Summarization}
% 	Structured data summarization is the task where natural language description is generated from a structured data input. The task requires content selection and surface realization. Content selection determines what parts of the input are to be chosen and surface realization describes the selected content into natural language text.\\
% 	Tabular data summarization is an important task of describing a table with header information into natural language. This is different from general structured data summarization tasks proposed (like wikipedia biographies , wikidata) , since , in this case multiple records are present for the same attributes, which demands selecting content in a hierarchical manner. Tabular data summarization where each instance can have different attributes or schema is an interesting problem both for academic and industrial use cases. However, given that there is large amount of tabular data generated from database systems and fixed format reports summarizing tables with fixed schema or attributes is clearly very useful to pursue. If schema is known then one could think of a template based system to generate natural langauge text. However, such an approach will not be scalable in terms of number of templates and will demand hand-crafted content selection rules. This motivated us to focus on summarizing tables with fixed/known attributes. We call such task of summarizing a table with fixed schema as standard table summarization. \\
% 	A table consist of set of records $ R = (r_{1}, r_{2},...r_{N})$ and each record has set of attributes $ A^{r} = (a_{1},a_{2},...a_{M})$. $U = (U_1, U_2,...U_N)$ represents the type of each record where $U_i$ is the record type for record $r_i$. Training data consist of instance pairs $(R_i, Y_i)$ for $i = 1,2,..n$, where $R_i$ represents the input table and $Y_i$ represents the corresponding natural language summary.

